LazyDAgger: Reducing Context Switching in Interactive Imitation Learning

Corrective interventions while a robot is learning to automate a task provide an intuitive method for a human supervisor to assist the robot and convey information about desired behavior. However, these interventions can impose significant burden on a human supervisor, as each intervention interrupts other work the human is doing, incurs latency with each context switch between supervisor and autonomous control, and requires time to perform. We present LazyDAgger, which extends the interactive imitation learning (IL) algorithm SafeDAgger to reduce context switches between supervisor and autonomous control. We find that LazyDAgger improves the performance and robustness of the learned policy during both learning and execution while limiting burden on the supervisor. Simulation experiments suggest that LazyDAgger can reduce context switches by an average of 60% over SafeDAgger on 3 continuous control tasks while maintaining state-of-the-art policy performance. In physical fabric manipulation experiments with an ABB YuMi robot, LazyDAgger reduces context switches by 60% while achieving a 60% higher success rate than SafeDAgger at execution time.

==> 0-macros.tex <==
%\usepackage{amsmath,graphics}
%\usepackage{amssymb} 
%\usepackage{nicefrac, multirow}
%\usepackage{algpseudocode}
%\usepackage[linesnumbered]{algorithm2e}
%\usepackage{tikz}
%\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}
%\usepackage{pgfplots}
% \pgfplotsset{compat=newest}
%\usepackage{subfig}
%\usepackage{textcomp}
%\usepackage{wrapfig}
\usetikzlibrary{backgrounds}
\numberwithin{equation}{section} 
%\newtheorem{thm}{Theorem}[section]  
%\newtheorem{cor}[thm]{Corollary}    % Corollary environment
%\newtheorem{lem}[thm]{Lemma}        % Lemma environment
%\newtheorem{dfn}[thm]{Definition}        % Lemma environment
%\newtheorem{prop}[thm]{Proposition}  % Proposition environment
%\newtheorem{rem}[thm]{Remark}  % Proposition environment
%\newtheorem{con}[thm]{Conjecture}  % Proposition environment
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\ceq}{\ensuremath{\mathrel{\stackrel{\mathrm{def}}{=}}}} 
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\rd}{{\mathrm d}}
\newcommand{\p}{\partial}
\tikzstyle{every node}=[font=\small]
%%\usepackage{filemod}
\newcommand{\includetikz}[2]{%
\tikzsetnextfilename{#2}%
    \filemodCmp{#1#2.tikz}{#1tikz/#2.pdf}%
        {\tikzset{external/remake next}}{}%
    \input{#1#2.tikz}%
}

\captionsetup{font={footnotesize}}

%\usepackage{tabularx}
%\usepackage{pbox}
%\usepackage{ragged2e}
%\usepackage{multirow}
%\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcolumntype{L}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\RaggedLeft\hspace{0pt}}p{#1}}

\DeclareMathOperator{\J}{J} 
\DeclareMathOperator{\clamp}{clamp} 
\DeclareMathOperator{\interior}{int} 
\DeclareMathOperator{\D}{D} 
\DeclareMathOperator{\Div}{div} 
\DeclareMathOperator{\Sgn}{Sgn} 
\DeclareMathOperator{\Hom}{Hom} 
\DeclareMathOperator{\rank}{rank} 
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\Area}{Area}
\DeclareMathOperator{\dVol}{dVol}
\DeclareMathOperator{\supp}{supp} 
\DeclareMathOperator{\Int}{Int} 
\DeclareMathOperator{\Conv}{Conv} 
\DeclareMathOperator{\Cone}{Cone} 
\DeclareMathOperator{\Ker}{Ker} 
\DeclareMathOperator{\Span}{Span} 
\DeclareMathOperator{\Min}{Min} 
\newcommand{\bone}{\mathbf{1}}
\DeclareMathOperator{\tr}{tr} 
\newcommand{\bR}{\mathbb{R}} 
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}} 
\newcommand{\bB}{\mathbb{B}} 
\newcommand{\bbT}{\mathbb{T}} 
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cO}{\mathcal{O}} 
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cKG}{\mathcal{KG}}
\renewcommand{\phi}{\varphi}
\renewcommand{\div}{\mbox{div}}
\newcommand{\ve}{\varepsilon}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\diff}[4]{\left.\left.\frac{\operatorname{d}}{\operatorname{d}#1}\right.^{#2}#3\right|_{#4}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\furlp}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/papers/#1.pdf}{D}}}
\newcommand{\furlb}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/books/#1.pdf}{D}}}
\newcommand{\fcitep}[1]{\cite{#1}\mbox{\furlp{#1}}}
\newcommand{\fciteb}[1]{\cite{#1}\mbox{\furlb{#1}}}
% we can now use cite as before
% misc defines
\newcommand{\energy}{U}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\hbx}{\hat{\mathbf{x}}}
\newcommand{\bbx}{\bar{\mathbf{x}}}
\newcommand{\sbx}{\mathbf{x}^{\star}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\hbb}{\hat{\mathbf{b}}}
\newcommand{\hbn}{\hat{\mathbf{n}}}
\newcommand{\bbb}{\bar{\mathbf{b}}}
\newcommand{\hbu}{\hat{\mathbf{u}}}
\newcommand{\bbu}{\bar{\mathbf{u}}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\hmX}{\hat{\mathcal{X}}}
\newcommand{\hmU}{\hat{\mathcal{U}}}
\newcommand{\bmX}{\bar{\mathcal{X}}}
\newcommand{\bmU}{\bar{\mathcal{U}}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\hbpsi}{\hat{\boldsymbol \psi}}
\newcommand{\bPsi}{\boldsymbol \Psi}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\sS}[1]{\sqrt{\Sigma_{#1}}}
\newcommand{\shS}[1]{\sqrt{\hat{\Sigma}_{#1}}}
\newcommand{\sd}{\texttt{sd}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\dt}{dt}
\DeclareMathOperator{\Vect}{vec}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\argmin}{arg\,min}

\newcommand{\specialcell}[2][c]{ \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\limit}[1] {\underset{#1}{\text{lim }}}
\newcommand{\infimum}[1] {\underset{#1}{\text{inf }}}
\newcommand{\supremum}[1] {\underset{#1}{\text{sup }}}
\newcommand{\maximum}[1] {\underset{#1}{\text{max }}}
\newcommand{\minimum}[1] {\underset{#1}{\text{min }}}
\newcommand{\myargmax}[1] {\underset{#1}{\text{argmax }}}
\newcommand{\myargmin}[1] {\underset{#1}{\text{argmin }}}
\newcommand{\expect}[1] {\mathbb{E}\left[#1\right]}

\newcommand{\TODO}[1]{\todo{#1}}



==> CASE 2021_ Lazy-DAgger/0-defs.tex <==
\usepackage{xspace}
\newcommand{\algname}{LazyDAgger\xspace}
\newcommand{\algabbr}{LazyDAgger\xspace}
\newcommand{\justalgname}{LazyDAgger\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\params}{\mathbf{\theta}}
\newcommand{\piparams}{\mathbf{\theta}_\pi}
\newcommand{\repparams}{\mathbf{\theta}_s}

\newcommand{\markov}{\mathcal{M}}
\newcommand{\state}{\mathbf{s}}
\newcommand{\tstate}{\mathbf{s}_t}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\action}{\mathbf{a}}
\newcommand{\taction}{\mathbf{a}_t}
\newcommand{\stateinitial}{\rho_0}
\newcommand{\rewardfn}{r}
% \newcommand{\gamma}{\gamma}
\newcommand{\transition}{\mathcal{T}}
\newcommand{\timemax}{T}
\newcommand{\policy}{\pi}

\newcommand{\cartdelta}{\Delta \mathbf{x}}
\newcommand{\cartpos}{\mathbf{x}}
\newcommand{\cartpost}{\mathbf{x}_t}
\newcommand{\cartposd}{\mathbf{x}_{\textrm{des}}}
\newcommand{\cartposdt}{\mathbf{x}_k}
\newcommand{\cartvel}{\mathbf{v}}
\newcommand{\cartveld}{\mathbf{v}_{\textrm{des}}}
\newcommand{\cartveldt}{\mathbf{v}_k}
\newcommand{\cartacc}{\mathbf{a}}
\newcommand{\cartaccd}{\mathbf{a}_{\textrm{des}}}
\newcommand{\cartaccdt}{\mathbf{a}_k}
\newcommand{\cartaccu}{\mathbf{a}_u}

\newcommand{\kp}{\mathbf{k}_{\textrm{p}}}
\newcommand{\kv}{\mathbf{k}_{\textrm{v}}}
\newcommand{\taurobot}{\mathbf{\tau}_{\textrm{u}}}


% notations
% math operators
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\indi}[1]{\mathbb{I}\left[#1\right]}

\newcommand{\chk}{\texttt{Inspect}}
\newcommand{\lbl}{\texttt{Label}}
\newcommand{\demo}{\texttt{HierDemo}}
\newcommand{\success}{\texttt{success}\xspace}
\newcommand{\terminal}{\texttt{terminal}\xspace}
\newcommand{\pseudo}{\texttt{pseudo}\xspace}%{\texttt{pseudo-reward}}
\newcommand{\reward}{\texttt{reward}\xspace}
\newcommand{\grasp}{\texttt{grasp}\xspace}
\newcommand{\push}{\texttt{push}\xspace}%{\texttt{pseudo-reward}}
\newcommand{\ptree}{\texttt{policy\_tree}\xspace}
\newcommand{\search}{\texttt{search}\xspace}
\newcommand{\singulate}{\texttt{singulate}\xspace}%{\texttt{pseudo-reward}}
\newcommand{\True}{\textit{True}}
\newcommand{\False}{\textit{False}}

% % POMDP
% \newcommand{\goals}{\mathcal{G}} % goals
% \newcommand{\states}{\ensuremath{\mathcal{S}}}
% \newcommand{\actions}{\ensuremath{\mathcal{A}}}
\newcommand{\transitions}{\ensuremath{\mathcal{T}}}
\newcommand{\rewards}{\ensuremath{\mathcal{R}}}
\newcommand{\observations}{\ensuremath{\mathcal{Y}}}
\newcommand{\observationprobs}{\ensuremath{\Upsilon}}
\newcommand{\tree}{\ensuremath{\mathcal{X}}}

\newcommand{\bp}{bp} % ?
\newcommand{\bx}{bx} % ?
\newcommand{\by}{by} % ?
\newcommand{\bu}{bu} % ?
\newcommand{\mC}{C} % ?

\newcommand{\Fig}[1]{Figure~\ref{fig:#1}}

\captionsetup{font={footnotesize}}

\newcommand{\limit}[1] {\underset{#1}{\text{lim }}}
\newcommand{\infimum}[1] {\underset{#1}{\text{inf }}}
\newcommand{\supremum}[1] {\underset{#1}{\text{sup }}}
\newcommand{\maximum}[1] {\underset{#1}{\text{max }}}
\newcommand{\minimum}[1] {\underset{#1}{\text{min }}}
%\newcommand{\pistarsafe} {\pi_{\rm S}^*}
% Daniel S: Prof Goldberg suggestions (March 13)
\newcommand{\ffilt} {f}
\newcommand{\fstarfilt} {f^*}
\newcommand{\cloningloss} {\mathcal{L}(\pi_{R}(s_t),\pi_{H}(s_t))}
\newcommand{\metaloss} {\rho_{H}}
\newcommand{\tausup} {\beta_{H}} % tau? textrm?
\newcommand{\tauauto} {\beta_{R}} % textrm auto?
\newcommand{\pisup} {\pi_{H}} 
\newcommand{\pirob} {\pi_{R}}
\newcommand{\pimeta} {\pi}
\newcommand{\indicatorint} {m_I} % Daniel S: is this what he wanted?
\newcommand{\indicatorsup} {m_H} % Daniel S: is this what he wanted?
\newcommand{\dsafe} {\mathcal{D}_{\rm S}} 
\newcommand{\lsafe} {\mathcal{L}_{\rm S}} 

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\expect}[1] {\mathbb{E}\left[#1\right]}

\newcommand{\TODO}[1]{\todo{#1}}
\newcommand{\brijen}[1]{{\color{red}Brijen: {#1}}}
\newcommand{\ashwin}[1]{{\color{blue}Ashwin: {#1}}}
\newcommand{\ryan}[1]{{\color{OliveGreen}Ryan: {#1}}}
\newcommand{\daniel}[1]{{\color{green}Daniel S: {#1}}}
\newcommand{\db}[1]{{\color{orange}DB: {#1}}}
\newcommand{\michael}[1]{{\color{cyan}Michael: {#1}}}


==> CASE 2021_ Lazy-DAgger/0-macros.tex <==
%\usepackage{amsmath,graphics}
%\usepackage{amssymb} 
%\usepackage{nicefrac, multirow}
%\usepackage{algpseudocode}
%\usepackage[linesnumbered]{algorithm2e}
%\usepackage{tikz}
%\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}
%\usepackage{pgfplots}
% \pgfplotsset{compat=newest}
%\usepackage{subfig}
%\usepackage{textcomp}
%\usepackage{wrapfig}
\usetikzlibrary{backgrounds}
\numberwithin{equation}{section} 
%\newtheorem{thm}{Theorem}[section]  
%\newtheorem{cor}[thm]{Corollary}    % Corollary environment
%\newtheorem{lem}[thm]{Lemma}        % Lemma environment
%\newtheorem{dfn}[thm]{Definition}        % Lemma environment
%\newtheorem{prop}[thm]{Proposition}  % Proposition environment
%\newtheorem{rem}[thm]{Remark}  % Proposition environment
%\newtheorem{con}[thm]{Conjecture}  % Proposition environment
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\ceq}{\ensuremath{\mathrel{\stackrel{\mathrm{def}}{=}}}} 
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\rd}{{\mathrm d}}
\newcommand{\p}{\partial}
\tikzstyle{every node}=[font=\small]
%%\usepackage{filemod}
\newcommand{\includetikz}[2]{%
\tikzsetnextfilename{#2}%
    \filemodCmp{#1#2.tikz}{#1tikz/#2.pdf}%
        {\tikzset{external/remake next}}{}%
    \input{#1#2.tikz}%
}

\captionsetup{font={footnotesize}}

%\usepackage{tabularx}
%\usepackage{pbox}
%\usepackage{ragged2e}
%\usepackage{multirow}
%\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcolumntype{L}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\RaggedLeft\hspace{0pt}}p{#1}}

\DeclareMathOperator{\J}{J} 
\DeclareMathOperator{\clamp}{clamp} 
\DeclareMathOperator{\interior}{int} 
\DeclareMathOperator{\D}{D} 
\DeclareMathOperator{\Div}{div} 
\DeclareMathOperator{\Sgn}{Sgn} 
\DeclareMathOperator{\Hom}{Hom} 
\DeclareMathOperator{\rank}{rank} 
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\Area}{Area}
\DeclareMathOperator{\dVol}{dVol}
\DeclareMathOperator{\supp}{supp} 
\DeclareMathOperator{\Int}{Int} 
\DeclareMathOperator{\Conv}{Conv} 
\DeclareMathOperator{\Cone}{Cone} 
\DeclareMathOperator{\Ker}{Ker} 
\DeclareMathOperator{\Span}{Span} 
\DeclareMathOperator{\Min}{Min} 
\newcommand{\bone}{\mathbf{1}}
\DeclareMathOperator{\tr}{tr} 
\newcommand{\bR}{\mathbb{R}} 
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}} 
\newcommand{\bB}{\mathbb{B}} 
\newcommand{\bbT}{\mathbb{T}} 
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cO}{\mathcal{O}} 
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cKG}{\mathcal{KG}}
\renewcommand{\phi}{\varphi}
\renewcommand{\div}{\mbox{div}}
\newcommand{\ve}{\varepsilon}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\diff}[4]{\left.\left.\frac{\operatorname{d}}{\operatorname{d}#1}\right.^{#2}#3\right|_{#4}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\furlp}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/papers/#1.pdf}{D}}}
\newcommand{\furlb}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/books/#1.pdf}{D}}}
\newcommand{\fcitep}[1]{\cite{#1}\mbox{\furlp{#1}}}
\newcommand{\fciteb}[1]{\cite{#1}\mbox{\furlb{#1}}}
% we can now use cite as before
% misc defines
\newcommand{\energy}{U}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\hbx}{\hat{\mathbf{x}}}
\newcommand{\bbx}{\bar{\mathbf{x}}}
\newcommand{\sbx}{\mathbf{x}^{\star}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\hbb}{\hat{\mathbf{b}}}
\newcommand{\hbn}{\hat{\mathbf{n}}}
\newcommand{\bbb}{\bar{\mathbf{b}}}
\newcommand{\hbu}{\hat{\mathbf{u}}}
\newcommand{\bbu}{\bar{\mathbf{u}}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\hmX}{\hat{\mathcal{X}}}
\newcommand{\hmU}{\hat{\mathcal{U}}}
\newcommand{\bmX}{\bar{\mathcal{X}}}
\newcommand{\bmU}{\bar{\mathcal{U}}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\hbpsi}{\hat{\boldsymbol \psi}}
\newcommand{\bPsi}{\boldsymbol \Psi}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\sS}[1]{\sqrt{\Sigma_{#1}}}
\newcommand{\shS}[1]{\sqrt{\hat{\Sigma}_{#1}}}
\newcommand{\sd}{\texttt{sd}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\dt}{dt}
\DeclareMathOperator{\Vect}{vec}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\argmin}{arg\,min}

\newcommand{\specialcell}[2][c]{ \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\limit}[1] {\underset{#1}{\text{lim }}}
\newcommand{\infimum}[1] {\underset{#1}{\text{inf }}}
\newcommand{\supremum}[1] {\underset{#1}{\text{sup }}}
\newcommand{\maximum}[1] {\underset{#1}{\text{max }}}
\newcommand{\minimum}[1] {\underset{#1}{\text{min }}}
\newcommand{\myargmax}[1] {\underset{#1}{\text{argmax }}}
\newcommand{\myargmin}[1] {\underset{#1}{\text{argmin }}}
\newcommand{\expect}[1] {\mathbb{E}\left[#1\right]}

\newcommand{\TODO}[1]{\todo{#1}}



==> CASE 2021_ Lazy-DAgger/0-preamble.tex <==
%%%%%%%%%%%% OLD PREAMBLE %%%%%%%%%%%%%%%%%

% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage[pdftex]{graphicx}
\usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200
\usepackage{epsfig}
\usepackage[font={small}]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
%\usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %special symbols
% \usepackage{amsfonts}
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations
% \usepackage{mathtools}
\numberwithin{equation}{section} 
\usepackage{dsfont}

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
% \DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

% \usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
% %should only use one of algorithmic or algorithmicx or algorithm2e
% % \usepackage{algorithmic} %least preferred
% % \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
% \usepackage{algorithmic} %algpseudocode:layout for algorithmicx

% \algtext*{EndFunction}% Remove "end while" text
% \algtext*{EndWhile}% Remove "end while" text
% \algtext*{EndIf}% Remove "end if" text


% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}
\usepackage{tabulary}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
% \usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
% \usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
\usepackage{balance} 
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{blindtext}

\let\labelindent\relax
\usepackage{enumitem}

% \usepackage{tikz}
% \usetikzlibrary{backgrounds}

\usepackage{ragged2e}
% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

% \usepackage[protrusion=true,expansion=true]{microtype}
% \setlength{\emergencystretch}{3em}

% \usepackage[yyyymmdd]{datetime}
% \renewcommand{\dateseparator}{-}
% \date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
\usepackage[usenames,dvipsnames,table,xcdraw]{xcolor}
\usepackage{pgfplots} %do not use with xcolor
\pgfplotsset{compat=newest}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}

%\usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
% \newcommand{\todo}[1]{\textcolor{red}{[#1?]}}
%takes in optional argument
\newcommand{\tocite}[1]{%
\textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
}

\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure\,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{1mm}        
\setlength{\belowcaptionskip}{0mm}        
\setlength{\textfloatsep}{0mm}
\setlength{\dbltextfloatsep}{3mm}
\renewcommand{\baselinestretch}{1.0}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother

\usepackage[pdfborder={0 0 0.5}]{hyperref}
% \usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=black,
    citecolor=black,
    filecolor=cyan,
    urlcolor=black
}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

\usepackage[switch]{lineno}

==> CASE 2021_ Lazy-DAgger/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% In environments with uncertain dynamics, learning-based control strategies have recently achieved success on many challenging robotic tasks~\cite{kroemer2019review,dexterous-manip, qt-opt, SAC-applications, DeepVisuomotor, pan2017agile, fabric_vsf}. Typically, these algorithms involve specifying objectives for robotic agents and then optimizing these objectives through model-based~\cite{fabric_vsf, dexterous-manip, DeepVisuomotor, SAVED, abc-lmpc} or model-free~\cite{rl-end-to-end, SAC-applications, qt-opt} control strategies. However, specifying reward functions can often lead to unintended consequences~\cite{ng1999policy,leike2018scalable,AI-safety, recovery-rl} or be too sparse or uninformative for a robot to successfully optimize~\cite{vecerik2017leveraging,overcoming_exploration}, leading to slow and inefficient learning~\cite{zhu2018reinforcement,SAVED}. 
Imitation learning allows a robot to learn from human feedback and examples~\cite{argall2009survey,arora2018survey,osa2018algorithmic}.
% Human examples and feedback can take many forms such as demonstrations~\cite{abbeel2004apprenticeship,overcoming_exploration,argall2009survey}, preferences~\cite{christiano2017deep,palan2019learning}, rankings~\cite{trex,brown2020safe}, action labels \cite{dagger,DART,brown2018risk}, kinesthetic corrections~\cite{bajcsy2017learning,losey2018review}, and reward and value signals~\cite{knox2009interactively,macglashan2017interactive,kessler2019active}.
In particular, \textit{interactive imitation learning} (IL)~\cite{EIL,hg_dagger,safe_dagger}, in which a human supervisor periodically takes control of the robotic system during policy learning, has emerged as a popular imitation learning method, as interventions are a particularly intuitive form of human feedback~\cite{EIL}. However, a key challenge in interactive imitation learning is to reduce the burden that interventions place on the human supervisor~\cite{safe_dagger, hg_dagger}.
%, since each intervention requires a human to allocate time towards helping the robot during learning. 

\begin{figure}[htb!]
\center
\includegraphics[width=0.49\textwidth]{figures/splash8.png}
\caption{
\algname learns to cede control to a supervisor in states in which it estimates that its actions will significantly deviate from those of the supervisor. \algname reduces context switches between supervisor and autonomous control to reduce burden on a human supervisor working on multiple tasks.}%(Bottom) Rollouts of SafeDAgger and \algname on a physical sequential fabric manipulation task consisting of smoothing a crumpled fabric, precisely aligning the corners, and folding. Human supervisor actions are indicated with red arrows while robot actions are indicated in green. \algname switches back to robot control when confident in task completion, while SafeDAgger ends human intervention prematurely, resulting in poor task performance and more context switches.}
%\vspace*{-10pt}
\label{fig:teaser}
\end{figure}

One source of this burden is the cost of \textit{context switches} between human and robot control. 
% Context switching provides both a critical cognitive challenge for human supervisors and a significant time cost. Research in cognitive science and computer science suggests context switching can be distracting, frustrating and time-consuming for humans~\cite{facebook_bleh_2013, multitasking_crazy_2008, fragmented_work_2005, interrupted_work_2004}. 
% Each context switch requires significant cognitive burden~\cite{gopher2000switching,rubinstein2001executive} and
Context switches incur significant time cost, as a human must interrupt the task they are currently performing, acquire control of the robot, and gain sufficient situational awareness before beginning the intervention. As an illustrative example, consider a robot performing a task for which an action takes 1 time unit and an intervention requires two context switches (one at the start and one at the end). We define \emph{latency} $L$ as the number of time units associated with a single context switch. For instance, $L \gg 1$ for a human supervisor who will need to pause an ongoing task and walk over to a robot that requires assistance. If the supervisor takes control 10 times for 2 actions each, she spends $20L + 20$ time units helping the robot. In contrast, if the human takes control 2 times for 10 actions each, she spends only $4L + 20$ time units. The latter significantly reduces the burden on the supervisor. Furthermore, prior work suggests that frequent context switches can make it difficult for the supervisor to perform other tasks in parallel~\cite{swamy2020scaled} or gain enough situational awareness to provide useful interventions~\cite{think_going}.

We present \algname (Figure~\ref{fig:teaser}), an algorithm which initiates useful interventions while limiting context switches.
% to efficiently use human interventions to learn reliable robotic control policies. 
The name \algname is inspired by the concept of lazy evaluation in programming language theory~\cite{lazy-eval}, where expressions are evaluated only when required to reduce computational burden. As in SafeDAgger~\cite{safe_dagger}, \algname learns a meta-controller which determines when to context switch based on the estimated discrepancy between the learner and supervisor. However, unlike SafeDAgger, \algname reduces context switching by (1) introducing asymmetric switching criteria and (2) injecting noise into the supervisor control actions to widen the distribution of visited states. One appealing property of this improved meta-controller is that even after training, \algname can be applied at execution time to improve the safety and reliability of autonomous policies with minimal context switching.
% Sustained interventions naturally reduce the frequency of context switches, while the noise injection procedure improves robustness in the learned robot policy. \algname can both (1) help the robot learn a more robust policy during training and (2) augment any deployed imitation learning policy to improve task performance as well as fine-tune the policy in continuous learning settings without excessive switching.
We find that across 3 continuous control tasks in simulation, \algname achieves task performance on par with DAgger~\cite{dagger} with 88\% fewer supervisor actions than DAgger and 60\% fewer context switches than SafeDAgger. In physical fabric manipulation experiments, we observe similar results, and find that at execution time, \algname achieves 60\% better task performance than SafeDAgger with 60\% fewer context switches. %\ashwin{TODO: @Ryan: update this paragraph to reflect new exp results?}






% These challenges are further exacerbated when a single human must control a fleet of robots
% There are three key elements to interactive IL algorithms: mechanisms to (1) \emph{initiate}, (2) \emph{collect}, and (3) \emph{learn from} interventions \ryan{reviewer 5 was confused by request vs collect}. While (1) and (3) have been studied extensively in prior work~\cite{safe_dagger,hg_dagger,brown2018risk,palan2019learning,ensemble_dagger,EIL}, there has been comparatively little focus on (2): designing methods to collect informative interventions once an intervention is initiated. While interventions are often information-rich and intuitive to provide, the context switching needed to provide them can be frustrating and time-consuming for humans. Each context switch requires significant cognitive burden~\cite{gopher2000switching,rubinstein2001executive} and makes it difficult for the supervisor to perform other tasks in parallel~\cite{swamy2020scaled} or gain enough situational awareness to provide useful interventions~\cite{think_going}. \ryan{add a bunch of citations to justify context switching = bad} We hypothesize that context switching is a major source of supervisor burden in interactive IL and present an algorithm that can reduce the frequency of these switches \ryan{instead of hypothesizing this we can justify with the citations in the previous sentence}. Experiments suggest that sustained, infrequent demonstrations that expose the supervisor to a diverse set of states in uncertain regions can accelerate learning efficiency while reducing supervisor burden.

% We present \algname (Figure~\ref{fig:teaser}), an algorithm that extends prior work in imitation learning via data aggregation~\cite{dagger, safe_dagger, hg_dagger}, to efficiently use human interventions to learn reliable robotic control policies. The name is inspired by the concept of lazy evaluation in programming language theory, where expressions are evaluated parsimoniously to reduce computational burden.  As in prior work from~\citet{safe_dagger}, \algabbr learns a meta-controller which determines when to context switch based on the estimated discrepancy between the learner and supervisor.  \algabbr additionally (1) encourages sustained interventions by enforcing that interventions continue until the learner and supervisor policies closely match and (2) injects noise into the supervisor controls to increase robustness in the learned controller. We find that across 3 continuous control tasks in simulation, \algname achieves task performance on par with DAgger with 12\% of its supervisor burden and 60\% fewer context switches than the best interactive IL baseline. In physical fabric folding experiments we observe similar results and find that \algname achieves 40\% better task performance than SafeDAgger with fewer context switches and supervisor actions. \ryan{add something about safe/more reliable deployment of learned policies and robot fleets, motivating LazyDAgger-Execution}
% in addition to reducing the number of interventions, \algabbr often results in improved task performance when compared with state-of-the-art interactive imitation learning algorithms \ashwin{insert details on exp results}.
% In \algabbr, we extend prior work by focusing on two observations: (1) thrashing between supervisor and autonomous policies is often undesirable in practice due to the cognitive burden and human errors that occur due to frequent context switching for the human supervisor~\cite{gopher2000switching,rubinstein2001executive} and the need to have the supervisor available to frequently assist which limits the amount of time the supervisor can perform other tasks~\cite{crandall2005validating,swamy2020scaled}, and (2) interventions are more beneficial if the supervisor is exposed to long sequences of more diverse states~\cite{dagger,DART}. To achieve this, like in prior work~\cite{safe_dagger}, \algabbr learns a meta-controller which determines when to solicit interventions based on the estimated discrepancy between the learner. However, unlike prior work, \algabbr (1) encourages lengthy interventions by enforcing that intervention continue until the supervisor actions and those the learner would take are very similar to each other, indicating that further intervention is unnecessary and (2) injects noise into the supervisor controls to increase robustness in the learned controller. We find that in addition to reducing the number of interventions, \algabbr often results in improved task performance and comparable numbers of requests for supervisor action queries, when compared with state-of-the-art interactive imitation learning algorithms \ashwin{insert details on exp results}.

% \algabbr learns a high-level meta-controller that determines when to solicit interventions based on the estimated discrepancy between the learner and the supervisor while ensuring that the interventions are sufficiently lengthy and visit a diverse enough set of states to be useful for policy learning. The key insight in \algabbr is to improve the  efficiency of human interventions by (1) learning to ask for help only when needed, (2) minimizing context switching and possible human error due to a lag in situational awareness of states~\cite{hg_dagger}, and (3) injecting noise into the supervisor's actions in order to obtain a richer set of supervisor action labels concentrated around areas of state space where the robot needs help. \algabbr can be flexibly used in conjunction with any policy with an appropriate policy improvement mechanism. We evaluate \algabbr on \todo{insert}. We find that in addition to reducing the number of interventions, \algabbr often results in improved task performance and comparable numbers of requests for supervisor action queries, when compared with state-of-the-art interactive imitation learning algorithms.





==> CASE 2021_ Lazy-DAgger/2-related-work.tex <==
\section{Background and Related Work}
\label{sec:related-work}
Challenges in learning efficiency and reward function specification have inspired significant interest in algorithms that can leverage supervisor demonstrations and feedback for policy learning.

\textbf{Learning from Offline Demonstrations: }
% Demonstrations for IL, RL, Classical Control
Learning from demonstrations~\cite{argall2009survey,osa2018algorithmic,arora2018survey} is a popular imitation learning approach, as it requires minimal supervisor burden: the supervisor provides a batch of offline demonstrations and gives no further input during policy learning. Many methods use demonstrations directly for policy learning~\cite{pomerleau1991efficient,ijspeert2013dynamical,paraschos2013probabilistic,torabi2018behavioral}, while others use reinforcement learning to train a policy using a reward function inferred from demonstrations \cite{abbeel2004apprenticeship,ziebart2008maximum,ho2016generative,brown2019drex,airl}. Recent work has augmented demonstrations with additional offline information such as pairwise preferences~\cite{browngoo2019trex,brown2020safe}, human gaze~\cite{gaze_saran}, and natural language descriptions~\cite{tung2018reward}. While offline demonstrations are often simple to provide, the lack of online feedback makes it difficult to address specific bottlenecks in the learning process or errors in the resulting policy due to covariate shift~\cite{dagger}.

% Learning from demonstrations has also been extensively explored in the reinforcement learning community to guide or accelerate learning~\cite{bignold2020conceptual,najar2020reinforcement,LearningMPC,abc-lmpc,SAVED, overcoming_exploration, dqfd, ddpgfd}. 

% Rather than learning from a fixed set of human demonstrations or preferences, active learning methods query the human for additional data throughout the learning process. 
%This motivates active learning methods such as DAgger~\cite{dagger}, 

\textbf{Learning from Online Feedback: }
Many policy learning algorithms' poor performance stems from a lack of online supervisor guidance, motivating active learning methods such as DAgger, which queries the supervisor for an action in every state that the learner visits~\cite{dagger}. While DAgger has a number of desirable theoretical properties, labeling every state is costly in human time and can be a non-intuitive form of human feedback~\cite{DART}. More generally, the idea of learning from action advice has been widely explored in imitation learning algorithms~\cite{converging-supervisors,SHIV,judah2011active,jauhri2020interactive}.
There has also been significant recent interest in active preference queries for learning reward functions from pairwise preferences over demonstrations~\cite{sadigh2017active,christiano2017deep,ibarz2018reward,palan2019learning,biyik2019asking,brown2020safe}. However, many forms of human advice can be unintuitive, since the learner may visit states that are significantly far from those the human supervisor would visit, making it difficult for humans to judge what correct behavior looks like without interacting with the environment themselves~\cite{EIL,reddy2018shared}.

\textbf{Learning from Supervisor Interventions: } There has been significant prior work on algorithms for learning policies from interventions. \citet{training_wheels, ac-teach} leverage interventions from suboptimal supervisors to accelerate policy learning, but assume that the supervisors are algorithmic and thus can be queried cheaply. \citet{recovery-rl, advantage_interventions, trial_no_error} also leverage interventions from algorithmic policies, but for constraint satisfaction during learning. \citet{hg_dagger, EIL, IARL, LAND, HITL, teaching-strats} instead consider learning from human supervisors and present learning algorithms which utilize the timing and nature of human interventions to update the learned policy. By giving the human control for multiple timesteps in a row, these algorithms show improvements over methods that only hand over control on a state-by-state basis~\cite{perf-eval-IL}. However, the above algorithms assume that the human is continuously monitoring the system to determine when to intervene, which may not be practical in large-scale systems or continuous learning settings~\cite{crandall2005validating,chen2014human,swamy2020scaled,kessler2019active}. Such algorithms also assume that the human knows when to cede control to the robot, which requires guessing how the robot will behave in the future. \citet{safe_dagger} and \citet{ensemble_dagger} present imitation learning algorithms SafeDAgger and EnsembleDAgger, respectively, to address these issues by learning to request interventions from a supervisor based on measures such as state novelty or estimated discrepancy between the learner and supervisor actions. These methods can still be sample inefficient, and, as we discuss later, often result in significant context switching.
% If the human is managing several robots at once, this will overly burden the human by causing too frequent context switching which can decrease human performance and impede situational awareness~\cite{chen2014human,gopher2000switching,rubinstein2001executive}. 
By contrast, \algabbr encourages interventions that are both easier to provide and more informative. To do this, \algname prioritizes (1) sustained interventions, which allow the supervisor to act over a small number of contiguous sequences of states rather than a large number of disconnected intervals, and (2) interventions which demonstrate supervisor actions in novel states to increase robustness to covariate shift in the learned policy.

==> CASE 2021_ Lazy-DAgger/3-problem-statement.tex <==
% \begin{figure*}[htb!]
% \center
% \includegraphics[width=0.75\textwidth]{figures/controlflow5.png}
% \caption{
% \textbf{\algname: }We illustrate the full control flow of \algname on a given timestep $t$. First, \algname queries the robot policy for an action $a_t$ and evaluates its current state under action discrepancy classifier $\ffilt$. If $\ffilt$ predicts an action discrepancy of at least $\tausup$ (i.e., $\ffilt \geq 0.5$) or \algname is in supervisor mode (Mode = $\textrm{Sup}$), then \algname queries an action $a^H_t$ from the supervisor and executes a noise-injected version $\tilde{a}^H_t$ in the environment. Otherwise, \algname executes action $a_t$ from the robot policy. Finally, if \algname executes $\tilde{a}^H_t$, \algname evaluates the true action discrepancy $\mathcal{L}(a_t, \tilde{a}^H_t)$ between $a_t$ and $\tilde{a}^H_t$. The mode for the next timestep is set to Autonomous mode if $\mathcal{L}(a_t, \tilde{a}^H_t) < \tauauto$ and Supervisor otherwise. 
% }
% \label{fig:control-flow}
% \end{figure*}
\section{Problem Statement}
\label{sec:prob-statement}
We consider a setting in which a human supervisor is training a robot to reliably perform a task. The robot may query the human for assistance, upon which the supervisor takes control and teleoperates the robot until the system determines that it no longer needs assistance. We assume that the robot and human policy have the same action space, and that it is possible to pause task execution while waiting to transfer control. We formalize these ideas in the context of prior imitation learning literature.

We model the environment as a discrete-time Markov decision process (MDP) $\mathcal{M}$ with states $s \in \mathcal{S}$, actions $a \in \mathcal{A}$, and time horizon $T$ \cite{puterman2014markov}. The robot does not have access to the reward function or transition dynamics of $\mathcal{M}$ but can cede control to a human supervisor, who executes some deterministic policy $\pisup: \mathcal{S} \to \mathcal{A}$. We refer to times when the robot is in control as \textit{autonomous mode} and those in which the supervisor is in control as \textit{supervisor mode}. 
%We model the environment as a discrete-time Markov decision process (MDP) $\mathcal{M}$ with states $s \in \mathcal{S}$, actions $a \in \mathcal{A}$, and time horizon $T$ \cite{puterman2014markov}. We consider the interactive imitation learning (IL) setting~\cite{hg_dagger}, where the robot does not have access to the reward function or transition dynamics of the MDP but has access to a supervisor. We assume the supervisor implicitly follows some deterministic policy $\pisup: \mathcal{S} \to \mathcal{A}$ and that the robot can request interventions from the supervisor. 
We minimize a surrogate loss function $J(\pirob)$ to encourage the robot policy $\pirob: \mathcal{S} \to \mathcal{A}$ to match that of the supervisor ($\pisup$):
\begin{align}
    \label{eq:IL-objective}
    J(\pirob) = \sum_{t=1}^{T} \mathds{E}_{s_t \sim d^{\pirob}_t} \left[\mathcal{L}(\pirob(s_t),\pisup(s_t))\right],
\end{align}
where $\mathcal{L}(\pirob(s),\pisup(s))$ is an action discrepancy measure between $\pirob(s)$ and $\pisup(s)$ (e.g., the squared loss or 0-1 loss), and $d^{\pirob}_t$ is the marginal state distribution at timestep $t$ induced by executing $\pirob$ in MDP $\mathcal{M}$.

In interactive IL we require a meta-controller $\pimeta$ that determines whether to query the robot policy $\pirob$ or to query for an intervention from the human supervisor policy $\pisup$; importantly, $\pimeta$ consists of both (1) the high-level controller which decides whether to switch between $\pirob$ and $\pisup$ and (2) the low-level robot policy $\pirob$. A key objective in interactive IL is to minimize some notion of supervisor burden. To this end, let $\indicatorint(s_t; \pimeta)$ be an indicator which records whether a context switch between autonomous ($\pirob$) and supervisor ($\pisup$) modes occurs at state $s_t$ (either direction). Then, we define $C(\pimeta)$, the expected number of context switches in an episode under policy $\pimeta$, as follows: ${C(\pimeta) = \sum_{t=1}^{T} \mathds{E}_{s_t \sim d^{\pimeta}_t} \left[ \indicatorint(s_t; \pimeta) \right]}$, where $d^{\pimeta}_t$ is the marginal state distribution at timestep $t$ induced by executing the meta-controller $\pimeta$ in MDP $\mathcal{M}$. %Furthermore, we define \emph{latency} $L > 0$ as the number of time units associated with a single context switch, where each time unit is the time it takes for the supervisor to execute a single action.
% \begin{align}
%     \label{eq:int-objective}
%     C(\pi) = \sum_{t=1}^{T} \mathds{E}_{s_t \sim d^\pi_t} \left[ \mathds{1}_{\textrm{int}}(s_t; \pi) \right]
% \end{align}
Similarly, let $\indicatorsup(s_t; \pimeta)$ indicate whether the system is in supervisor mode at state $s_t$. We then define $D(\pimeta)$, the expected number of supervisor actions in an episode for the policy $\pimeta$, as follows: ${D(\pimeta) = \sum_{t=1}^{T} \mathds{E}_{s_t \sim d^\pimeta_t} \left[ \indicatorsup(s_t; \pimeta) \right]}$.
% \begin{align}
%     \label{eq:act-objective}
%     D(\pi) = \sum_{t=1}^{T} \mathds{E}_{s_t \sim d^\pi_t} \left[ \mathds{1}_{\textrm{sup}}(s_t; \pi) \right]
% \end{align}

We define \emph{supervisor burden} $B(\pimeta)$ as the expected time cost imposed on the human supervisor. This can be expressed as the sum of the expected total number of time units spent in context switching and the expected total number of time units in which the supervisor is actually engaged in performing interventions:% Stated precisely, we define \emph{supervisor burden} $B(\pimeta)$ as follows:
\begin{align}
    \label{eq:burden}
        B(\pimeta) = L \cdot C(\pimeta) + D(\pimeta),
\end{align}
where $L$ is context switch latency (Section~\ref{sec:introduction}) in time units, and each time unit is the time it takes for the supervisor to execute a single action. The learning objective is to find a policy $\pimeta$ that matches supervisor performance, $\pisup$, while limiting supervisor burden to lie within a threshold $\Gamma_{\rm b}$, set by the supervisor to an acceptable tolerance for a given task. To formalize this problem, we propose the following objective: 
\begin{align}
\begin{split}
    \label{eq:LazyDAgger-objective}
    \pimeta &= \argmin_{\pimeta' \in \Pi}\{ J(\pirob')
    \mid B(\pimeta') \leq \Gamma_{\rm b}\},
\end{split}
\end{align}
where $\Pi$ is the space of all meta-controllers, and $\pirob'$ is the low-level robot policy associated with meta-controller $\pimeta'$. 
% In Section~\ref{sec:prelims} we discuss the specifics of the meta-controller $\pimeta$ used in SafeDAgger~\cite{safe_dagger} and in Section~\ref{sec:alg} we present the one we use in \algname.
% \begin{align}
% \begin{split}
%     \label{eq:LazyDAgger-objective}
%     \pi &= \argmin_{\pi \in \Pi}\{ J(\pi)
%     \mid C(\pi) \leq \Gamma_{\rm int} \text{, } D(\pi) \leq \Gamma_{\rm sup}\}
% \end{split}
% \end{align}

% This captures the intuition that the number of switches in control between the learner and the supervisor and the number of actions in supervisor mode approximately measure the online burden inflicted by \algname on the supervisor.
% \ashwin{Prof mentioned adding number of actions into this objective as well, still thinking about best way to do this}
% \ashwin{Will add an explicit term on minimizing switches tonight}
% In our work, we seek to minimize both the surrogate loss as well minimize the number of supervisor interventions. %I wonder if we should actually make this an explicit objective?

% We consider robotic control under Markov decision processes (MDPs), which can be described by the tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, P(\cdot|\cdot,\cdot), R(\cdot, \cdot), \gamma, \mu)$, where $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces.
% The stochastic dynamics model $P: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow [0, 1]$ maps a state and action to a probability distribution over subsequent states, $\gamma \in [0, 1]$ is a discount factor, $\mu$ is the initial state distribution ($s_0\sim\mu$), and $R: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function.

% Let $\Pi$ be the set of deterministic, Markovian policies $\pi: \mathcal{S} \rightarrow \mathcal{A}$. Given policy $\pi \in \Pi$, the expected return is defined as $R^\pi = \mathbb{E}_{\pi,\mu, P}\left[ \sum_t \gamma^t R(s_t, a_t)\right]$. The objective of \algabbr is to solve the following constrained optimization problem:
% \begin{align}
% \label{eq:objective}
%     \pi^* = \argmax_{\pi \in \Pi} \{R^\pi\}
% \end{align}
% We assume access to a potentially suboptimal supervisor policy $\pi_{\text{sup}}$ that can be queried online, where $R^{\pi_{\text{sup}}} \leq R^{\pi^*}$. We also assume that the supervisor is able to take over control safely and indicate actions $a \in \mathcal{A}$. For example, a human supervisor can easily indicate a pick-and-place action via a user interface, but may not be able to help with tasks involving extremely high-frequency control or high-dimensional control inputs. The objective is to learn a policy $\pi$ that best approximates $\pi_{\text{sup}}$.

% In the \textit{reinforcement learning} setting, we have access to a reward function and we seek to learn $\pi^\star$, which may obtain higher expected return than $\pi_{\text{sup}}$.

\section{Preliminaries: SafeDAgger}
\label{sec:prelims}
% The goal of imitation learning is to learn a policy $\pi$ to match the trajectory distribution of a supervisor $\pi_{\text{sup}}$ as closely as possible. More precisely, in imitation learning, the robot typically does not have access to any specified objective or reward function, but instead attempts to minimize a surrogate loss function which measures the discrepancy between the learner's policy $\pi$ and the supervisor $\pi_{\text{sup}}$~\cite{dagger}. Precisely, the learner solves the following optimization problem:
% \begin{align}
%     \label{eq:IL-objective}
%     \pi = \argmin_{\pi \in \Pi} \mathds{E}_{s \sim d_\pi} \left[L(\pi(s),\pi_{\rm sup}(s))\right]
% \end{align}
% where $L(\pi(s),\pi_{\rm sup}(s))$ is an action discrepancy measure between $\pi(s)$ and $\pi_{\text{sup}}(s)$ (squared loss, 0-1 loss, etc.).  and $d_\pi$ is the marginal state distribution induced by executing \textit{the learner policy} $\pi$ in MDP $\mathcal{M}$.
% One popular approach for optimizing the imitation learning objective is Behavior Cloning~\cite{pomerleau1991efficient,osa2018algorithmic}, which optimizes Equation~\eqref{eq:IL-objective} over a static dataset of offline trajectories collected from $\pi_{\text{sup}}$. However, this approach suffers from poor performance due to distribution mismatch~\cite{dagger}: the learner trains on samples from $d_{\pi_{\text{sup}}}$ but encounters trajectories from $d_{\pi}$ during execution. One popular approach to address these challenges both in theory and practice is DAgger~\cite{dagger}, which optimizes Equation~\eqref{eq:IL-objective} over an aggregated dataset of trajectories from $\pi$ and action labels from $\pi_{\text{sup}}$ for each state in the dataset. While this aggregation scheme results in desirable regret bounds~\cite{dagger}, providing action labels offline can often be highly non-intuitive~\cite{DART, SHIV, hg_dagger} and error prone~\cite{chuck2017cleaning}, making DAgger difficult to use in practice.
We consider interactive IL in the context of the objective introduced in Equation~\eqref{eq:LazyDAgger-objective}: to maximize task reward while limiting supervisor burden. To do this, \algabbr builds on SafeDAgger~\cite{safe_dagger}, a state-of-the-art algorithm for interactive IL. SafeDAgger selects between autonomous mode and supervisor mode by training a binary action discrepancy classifier $\ffilt$ to discriminate between ``safe" states which have an action discrepancy below a threshold $\tausup$ (i.e., states with ${\mathcal{L}(\pirob(s), \pisup(s)) < \tausup}$) and ``unsafe" states (i.e. states with ${\mathcal{L}(\pirob(s), \pisup(s)) \geq \tausup}$). The classifier $\ffilt$ is a neural network with a sigmoid output layer (i.e., $\ffilt(s) \in [0, 1]$) that is trained to minimize binary cross-entropy (BCE) loss on the datapoints $(s_t,\pisup(s_t))$ sampled from a dataset $\mathcal{D}$ of trajectories collected from $\pisup$. This is written as follows:
\begin{align}
\label{eq:safe-loss}
    \begin{split}
    \lsafe(\pirob(s_t),\pisup(s_t), \ffilt) 
    = -\fstarfilt(\pirob(s_t),\pisup(s_t))\log \ffilt(s_t) \\
    -(1 - \fstarfilt(\pirob(s_t), \pisup(s_t)))\log (1 - \ffilt(s_t) ),
    \end{split}
\end{align}
where the training labels are given by $\fstarfilt(\pirob(s_t),\pisup(s_t)) = \mathbbm{1}\left\{\mathcal{L}(\pirob(s_t), \pisup(s_t)) \geq  \tausup\right\}$, and $\mathbbm{1}$ denotes the indicator function.
Thus, $\lsafe(\pirob(s_t),\pisup(s_t),\ffilt)$ penalizes incorrectly classifying a ``safe" state as ``unsafe" and vice versa. %a binary cross-entropy loss function on the target distribution $\fstarfilt(\pirob(s_t),\pisup(s_t))$ and predicted distribution $\ffilt(s_t)$.

SafeDAgger executes the meta-policy $\pimeta$ which selects between $\pirob$ and $\pisup$ as follows:
\begin{align}
    \label{eq:safe_dagger_policy}
    \pimeta(s_t) =\begin{cases}
            \pirob(s_t) \text{ if } \ffilt(s_t) < 0.5 \\
            \pisup(s_t) \text{ otherwise},
          \end{cases}
\end{align}
 %\brijen{I think the first case should be $\geq 1/2$, or some thresh the way it's written above, since $\ffilt$ outputs values from $(0,1)$}
where $f(s_t) < 0.5$ corresponds to a prediction that $\mathcal{L}(\pirob(s_t), \pisup(s_t)) < \tausup$, i.e., that $s_t$ is ``safe.'' Intuitively, SafeDAgger only solicits supervisor actions when $\ffilt$ predicts that the action discrepancy between $\pirob$ and $\pisup$ exceeds the safety threshold $\tausup$. Thus, SafeDAgger provides a mechanism for querying the supervisor for interventions only when necessary. In \algabbr, we utilize this same mechanism to query for interventions but enforce new properties once we enter these interventions to lengthen them and increase the diversity of states observed during the interventions.
% \begin{align}
% \label{eq:bc-loss}
% L_{BC}(D, \pi) = \frac{1}{N} \sum_{i=1}^{N} ||\pi(s_i) - a_i||_2^2
% \end{align}
%  where $N$ is the total number of $(s_i, a_i)$ tuples in our dataset $D$. Our learned policy is $$ \pi = \arg\min_{\pi}{L(D, \pi)} $$
% \subsection{Imitation Learning with Dataset Aggregation (DAgger)}
% Unfortunately, in practice Behavior Cloning gives a very brittle policy due to compounding errors as soon as the learner leaves the supervisor's distribution \cite{dagger}. To mitigate this, one popular strategy is Dataset Aggregation (DAgger) \cite{dagger}, which provides more information on the learner's distribution. After training on the initial offline dataset $D$, we run our learned policy in the environment and collect its trajectories: $\{(s_0, \pi(s_0)), (s_1, \pi(s_1)), \dots\}$. We relabel each of these visited states $\{s_i\}$ online with what the \textit{supervisor} would have done at that state, giving us a new dataset $D' = \{(s_0, \pi_{\text{sup}}(s_0)), (s_1, \pi_{\text{sup}}(s_1)), \dots\}$. We then aggregate this new dataset $D'$ with our existing one ($D = D \cup D'$) and repeat the process for a fixed number of iterations. While this technique combats distribution shift, labeling each state online can be a very burdensome process that scales poorly, especially for a human supervisor.
% \subsection{SafeDAgger}
% To mitigate these issues, several works seek to reduce the burden on the supervisor \cite{SHIV, DART, safe_dagger}. Of these, the most similar to our approach is SafeDAgger~\cite{safe_dagger}. To deal with potential safety issues and reduce supervisor burden, SafeDAgger trains a classifer $\pi_{\text{safe}}$ to discriminate between ``safe" states (i.e. states with predicted action discrepancy below some predefined threshold $\tau$) and ``unsafe" states by optimizing the following binary cross-entropy loss:
% \begin{align}
% \label{eq:safe-loss}
%     L_{\textrm{safe}}(D,\pi, \pi_{\textrm{safe}}) 
%     = -\frac{1}{N} \sum_{i=1}^{N}(\pi_{\text{safe}}^*(s_i,a_i,\pi)\log \pi_{\text{safe}}(s_i) \\
%     +(1 - \pi_{\text{safe}}^*(s_i,a_i,\pi))\log (1 - \pi_{\text{safe}}(s_i) ))
% \end{align}

% where $$ \pi_{\text{safe}}^*(s_i, a_i, \pi) = \begin{cases} 1 \text{ if } ||\pi(s_i)-a_i||_2^2 \leq \tau \\ 0 \text{ otherwise } \end{cases} $$ and $\pi$ is our imitation learner. When the classifier believes the state is unsafe, it lets the supervisor control the system instead, and only collects training examples when the supervisor is in control. SafeDAgger demonstrates a significant reduction in supervisor burden and provides a mechanism that can extend to test-time policy deployment. However, they do not consider the supervisor burden involved in taking over control and relinquishing control, resulting in very frequent interventions that often last only one time-step long. In contrast, we seek to reduce supervisor burden in terms of both overall number of actions provided as well as the number of interventions, as the effort required to provide an additional action once already in control is often much less than that of assuming control of the system.
% \subsection{Reinforcement Learning}
% While many proposed improvements to DAgger \cite{safe_dagger, hg_dagger, dropout_dagger, SHIV, DART} solely evaluate their methods in the imitation learning setting, we observe that our \algabbr framework is agnostic to the implementation of the learner as long as it is able to incorporate the information that the supervisor provides. One such implementation is reinforcement learning, which has been shown to benefit from demonstrations \cite{overcoming_exploration, ddpgfd, ac-teach}, especially in sparse reward settings. In reinforcement learning, the goal is to learn a policy that maximizes the expected sum of discounted rewards in our MDP, i.e. $\mathbb{E}[\sum_t \gamma^t R(s_t, a_t)]$. In this setting, the robot typically does not have access to a supervisor policy, but it does have access to the reward at the states that it visits. As learning from scratch is inherently difficult, reinforcement learning has notoriously high sample complexity, has trouble dealing with exploration \cite{overcoming_exploration}, and can be brittle when deployed on physical systems. \algabbr may mitigate these issues by providing access to expert interventions when the learner needs help.

% We introduce a simple method to issue requests for supervisor intervention which is compatible with any off-policy control algorithm. The key insight is that interventions are likely to be useful in regions in which the robotic control policy and the supervisor are \emph{inconsistent}, and are otherwise likely unnecessary. Thus, like \todo{cite Safe DAgger}, we train a discrepancy estimator which estimates the divergence between the action chosen by the control policy and the supervisor without querying the supervisor. In \todo{cite Safe DAgger}, human action labels are solicited on states for which this discrepancy is sufficiently high. In contrast, when this discrepancy is sufficiently high, we request a supervisor intervention which is active until this discrepancy is no longer high again. This allows the robot to obtain sufficient experience in regions of the state space in which it is likely to diverge from the supervisor without relying on the supervisor to reliably label data outside of their data distribution.

% As in Safe DAgger we define a discrepancy measure between the learner and supervisor as follows:
% \begin{align}
%     \label{eq:discrep}
%     d(\pi, \pi^*, s) = \lVert \pi(s) - \pi^*(s) \rVert^2
% \end{align}
% We use this to define an intervention policy $\pi_I$ as follows ($1$ if should intervene, $0$ otherwise):
% \begin{align}
% \label{eq:intervene}
%     \pi_I(\pi, s) = \begin{cases}
%         1,    \   d(\pi, \pi^*, s) > \tau\\
%         0, \  \textrm{otherwise}
%     \end{cases}
% \end{align}
% Thus, $\pi_I$ can be used to determine when the $\pi$ and $\pi^*$ will diverge significantly without querying the $\pi^*$. The rest of the algorithm is functionally the same as Safe DAgger, but interventions are solicited instead of single actions when $\pi_I$ determines an intervention is required and you switch back the discrepancy between the supervisor and the robot is sufficiently low. No labeling so can use it with any control algorithm you wish. Tbh would be nice to consider this with model-based, model-free RL + IL as this would show the generality of the method and best distinguish it from Safe DAgger.

\begin{figure}[b!]
\center
\includegraphics[width=\linewidth]{figures/hyst2.png}
\caption{
\textbf{\algname Switching Strategy:  }SafeDAgger switches between supervisor and autonomous mode if the predicted action discrepancy is above threshold $\tausup$. In contrast, \algname uses asymmetric switching criteria and switches to autonomous mode based on ground truth action discrepancy. The gap between $\tauauto$ and $\tausup$ defines a hysteresis band~\cite{hysteresis}.}% This encourages lengthier interventions which reduce context switching between supervisor and autonomous modes, thereby reducing supervisor burden.}
\label{fig:hyst}
\end{figure}

==> CASE 2021_ Lazy-DAgger/4-methods.tex <==
\section{\algname}
\label{sec:alg}
%\algabbr is a new interactive IL algorithm which learns to request informative interventions to enable efficient policy learning while reducing context switches. Similar to SafeDAgger, \algabbr trains a classifier $\ffilt$ to determine when to request supervisor interventions. However, while SafeDAgger thresholds the output of this classifier to determine whether the learner ($\pi$) or supervisor ($\pisup$) is in control at each timestep, \algabbr explicitly reasons about whether it is in supervisor or autonomous mode, which makes it possible to encourage lengthy interventions (Section~\ref{subsec:ac-disc}) which expose the supervisor to a diverse set of states (Section~\ref{subsec:noise-inj}).

\begin{figure*}[htb!]
\center
\includegraphics[width=0.92\textwidth]{figures/mujocov6.png}
\caption{
\textbf{MuJoCo Simulation Results: }We study task performance (A), ablations (B), online supervisor burden (C), and total bidirectional context switches (D) for \algname and baselines over 3 random seeds. For Columns (A)-(D), the x-axis for all plots shows the number of epochs over the training dataset, while the y-axes indicate normalized reward (A, B), counts of supervisor actions (C, log scale), and context switches (D) with shading for 1 standard deviation. We find that \algname outperforms all baselines and ablations, indicating that encouraging lengthy, noisy interventions improves performance. Additionally, \algname uses far fewer context switches than other baselines while requesting far fewer supervisor actions than DAgger.}
\label{fig:mujoco}
\end{figure*}

\begin{algorithm}[t]
\caption{\algname}
\label{alg:main}
\footnotesize
\begin{algorithmic}[1]
\Require Number of epochs $N$, time steps per epoch $T$, intervention thresholds $\tausup$, $\tauauto$, supervisor policy $\pisup$, noise $\sigma^2$ %\ryan{add control flow for Execution Time?}
\State Collect ${\mathcal{D}}, \dsafe$ offline with supervisor policy $\pisup$
\State $\pirob \leftarrow \arg\min_{\pirob} \mathbb{E}_{(s_t, \pisup(s_t))\sim\mathcal{D}}\left[\cloningloss\right]$ \Comment{Eq.~\eqref{eq:IL-objective}}
\State $\ffilt \leftarrow \arg\min_{\ffilt} \mathbb{E}_{(s_t, \pisup(s_t))\sim\mathcal{D}\cup\dsafe} \left[\lsafe(\pirob(s_t),\pisup(s_t),\ffilt)\right]$ \Comment{Eq.~\eqref{eq:safe-loss}}
% \State Pretrain $\pirec$ and $\qsafehat$ on $\demos$ \Comment{Section~\ref{subsec:offline-pretraining}}
% \State $\mathcal{D}_{\mathrm{task}} \leftarrow \emptyset$, $\mathcal{D}_{\mathrm{rec}} \leftarrow \demos$
% \State $s_0 \leftarrow \texttt{env.reset()}$
\For{$i \in \{1,\ldots N\}$}
    \State Initialize $s_0$, Mode $\gets$ Autonomous
    \For{$t \in \{1,\ldots T\}$}
        \State $a_t \sim \pirob(s_t)$
        \If{Mode = Supervisor or $\ffilt(s_t) \geq 0.5$}
            \State $a^H_t = \pisup(s_t)$
            \State $\mathcal{D} \leftarrow \mathcal{D} \cup \{(s_t, a_t^H)\}$
            \State Execute $\tilde{a}^H_t \sim \mathcal{N}(a^H_t,\sigma^2I)$ \label{lin:noise}
            \If {$\mathcal{L}(a_t, a^H_t) < \tauauto$}
                \State Mode $\gets$ Autonomous
            \Else
                \State Mode $\gets$ Supervisor
            \EndIf
        \Else
            \State Execute $a_{t}$
        \EndIf
    \EndFor
    \State $\pirob \leftarrow \arg\min_{\pirob} \mathbb{E}_{(s_t, \pisup(s_t))\sim\mathcal{D}}\left[\cloningloss\right]$
    \State $\ffilt \leftarrow \arg\min_{\ffilt} \mathbb{E}_{(s_t, \pisup(s_t))\sim \mathcal{D}\cup \dsafe}\left[\lsafe(\pirob(s_t),\pisup(s_t),\ffilt)\right]$
\EndFor
\end{algorithmic}
\end{algorithm}
% \end{minipage}
% \vspace{-0.2in}
% \end{wrapfigure}

We summarize \algabbr in Algorithm~\ref{alg:main}. In the initial phase (Lines 1-3), we train $\pirob$ and safety classifier $\ffilt$ on offline datasets collected from the supervisor policy $\pisup$. In the interactive learning phase (Lines 4-19), we evaluate and update the robot policy for $N$ epochs, ceding control to the supervisor when the robot predicts a high action discrepancy.

\subsection{Action Discrepancy Prediction}
\label{subsec:ac-disc}
SafeDAgger uses the classifier $\ffilt$ to select between $\pirob$ and $\pisup$ (Equation~\eqref{eq:safe_dagger_policy}). However, in practice, this often leads to frequent context switching (Figure~\ref{fig:mujoco}). %A key design goal in \algabbr is to reduce context switches to inflict lower supervisor burden while also ensuring that each intervention is lengthy enough to be informative. 
To mitigate this, we make two observations. First, we can leverage that in supervisor mode, we directly observe the supervisor's actions. Thus, there is no need to use $\ffilt$, which may have approximation errors, to determine whether to remain in supervisor mode; instead, we can compute the ground-truth action discrepancy $\cloningloss$ exactly for any state $s_t$ visited in supervisor mode by comparing the supplied supervisor action $\pisup(s_t)$ with the action proposed by the robot policy $\pirob(s_t)$. In contrast, SafeDAgger uses $\ffilt$ to determine when to switch modes both in autonomous and supervisor mode, which can lead to very short interventions when $\ffilt$ prematurely predicts that the agent can match the supervisor's actions. Second, to ensure the robot has returned to the supervisor's distribution, the robot should only switch back to autonomous mode when the action discrepancy falls below a threshold $\tauauto$, where $\tauauto < \tausup$. %Thus, as in SafeDAgger, we solicit supervisor interventions when $\ffilt(s_t)$ predicts an action discrepancy greater than $\tausup$ (i.e. $\ffilt(s_t) \geq 0.5$), but the supervisor continues acting in the environment until the action discrepancy is sufficiently low (i.e. ${\cloningloss < \tauauto}$). 
As illustrated in Figure~\ref{fig:hyst}, \algname's asymmetric switching criteria create a hysteresis band, as is often utilized in control theory~\cite{hysteresis}. Motivated by Eq.~\eqref{eq:LazyDAgger-objective}, we adjust $\tausup$ to reduce context switches $C(\pimeta)$ and adjust $\tauauto$ as a function of $\tausup$ to increase intervention length. We hypothesize that redistributing the supervisor actions into fewer but longer sequences in this fashion both reduces burden on the supervisor and improves the quality of the online feedback for the robot. Details on setting these hyperparameter values in practice, the settings used in our experiments, and a hyperparameter sensitivity analysis are provided in the Appendix.% keeping the expected number of intervention actions $D(\pimeta)$ low. %The relative settings of $\tausup$ and $\tauauto$ are a function of the latency $L$. The larger $L$ is, the smaller $\tauauto$ should be set relative to $\tausup$ to encourage lengthier interventions which avoid frequent context switches. %While $\tausup$ and $\tauauto$ are tunable hyperparameters that vary with the task (see the Appendix), we can initialize $\tausup = \tauauto$ to the value that classifies approximately 25\% of the initial dataset $\mathcal{D} \cup \dsafe$ as unsafe, as in~\citet{safe_dagger}.

% \begin{figure}[t]
% \center
% \includegraphics[width=0.45\textwidth]{figures/mujocohistv4.png}
% \caption{
% \textbf{Intervention Length Distribution: } We compare the lengths of interventions between \algname and SafeDAgger on the MuJoCo environments using box and whisker plots. While almost all of SafeDAgger's interventions are very short, \algname takes longer interventions while still using a similar number of supervisor actions (see Figure~\ref{fig:mujoco}). Most of SafeDAgger's interventions are a single time step.}
% \label{fig:interventionhist}
% \end{figure}

%\vspace{0.2in}
\subsection{Noise Injection}
\label{subsec:noise-inj}
If the safety classifier is querying for interventions at state $s_t$, then the robot either does not have much experience in the neighborhood of $s_t$ or has trouble matching the demonstrations at $s_t$. This motivates exploring novel states near $s_t$ so that the robot can receive maximal feedback on the correct behavior in areas of the state space where it predicts a large action discrepancy from the supervisor. Inspired by prior work that has identified noise injection as a useful tool for improving the performance of imitation learning algorithms (e.g.~\citet{DART} and~\citet{brown2019drex}), we diversify the set of states visited in supervisor mode by injecting isotropic Gaussian noise into the supervisor's actions, where the variance $\sigma^2$ is a scalar hyperparameter (Line \ref{lin:noise} in Algorithm~\ref{alg:main}).
% \vspace{-0.13in}

%\subsection{Algorithm Overview}
%We provide an overview of \algabbr in Algorithm~\ref{alg:main}. As in SafeDAgger, \algname first uses $\pisup$ to collect offline datasets $\mathcal{D}$ and $\dsafe$, where the former is used to train the initial learner ($\pirob$) and both are used to train the initial action discrepancy classifier $\ffilt$.


==> CASE 2021_ Lazy-DAgger/5-results.tex <==
\section{Experiments}
\label{sec:results}
\begin{figure*}[htb!]
\center
\includegraphics[width=0.85\textwidth]{figures/sim2sim2.png}
\caption{
\textbf{Fabric Smoothing Simulation Results:} We study task performance measured by final fabric coverage (A), total supervisor actions (B), and total context switches (C) for \algname and baselines in the Gym-Cloth environment from~\cite{seita_fabrics_2020}. The horizontal dotted line shows the success threshold for fabric smoothing. \algname achieves higher final coverage than Behavior Cloning and SafeDAgger with fewer context switches than SafeDAgger but more supervisor actions. At execution time, we again observe that \algname achieves similar coverage as SafeDAgger but with fewer context switches.}
\label{fig:sim2sim}
\end{figure*}
We study whether \algname can (1) reduce supervisor burden while (2) achieving similar or superior task performance compared to prior algorithms. Implementation details are provided in the supplementary material. In all experiments, $\mathcal{L}$ measures Euclidean distance.  % on policy architectures, training procedures, and other experimental parameters in the supplementary material.

\subsection{Simulation Experiments: MuJoCo Benchmarks}\label{ssec:mujoco-results}
\textbf{Environments: }We evaluate \algname and baselines on 3 continuous control environments from MuJoCo~\cite{mujoco}, a standard simulator for evaluating imitation and reinforcement learning algorithms. In particular, we evaluate on HalfCheetah-v2, Walker2D-v2 and Ant-v2.
% which have state space sizes $|S| \in (17,17,111)$ and action space sizes $|A| \in (6,6,8)$ respectively.

\textbf{Metrics:}
\label{ssec:metrics}
For \algname and all baselines, we report learning curves which indicate how quickly they can make task progress in addition to metrics regarding the burden imposed on the supervisor. To study supervisor burden, we report the number of supervisor actions, the number of context switches, and the total supervisor burden (as defined in Eq.~\eqref{eq:burden}). Additionally, we define $L^* \geq 0$ to be the latency value such that for all $L > L^*$, \algname has a lower supervisor burden than SafeDAgger. We report this $L^*$ value, which we refer to as the \textit{cutoff latency}, for all experiments to precisely study the types of domains in which \algname is most applicable.

\textbf{Baselines:}
\label{ssec:baselines}
We compare \algname to Behavior Cloning~\cite{torabi2018behavioral}, DAgger~\cite{dagger}, and SafeDAgger~\cite{safe_dagger} in terms of the total supervisor burden and task performance. The Behavior Cloning and DAgger comparisons evaluate the utility of human interventions, while the comparison to SafeDAgger, another interactive IL algorithm, evaluates the impact of soliciting fewer but longer interventions.

\textbf{Experimental Setup: }For all MuJoCo environments, we use a reinforcement learning agent trained with TD3~\cite{td3} as an algorithmic supervisor. 
% On the HalfCheetah, Walker2D, and Ant environments, the supervisors obtain a reward of $5331 \pm 118$, $3492 \pm 1110$, and $4493 \pm 1580$ respectively.
We begin all \algabbr, SafeDAgger, and DAgger experiments by pre-training the robot policy with Behavior Cloning on 4,000 state-action pairs for 5 epochs, and similarly report results for Behavior Cloning after the 5th epoch. To ensure a fair comparison, Behavior Cloning uses additional offline data equal to the average amount of online data seen by \algabbr during training. All results are averaged over 3 random seeds.
%to control for stochasticity in training. 

\textbf{Results: }In Figure~\ref{fig:mujoco}, we study the performance of \algabbr and baselines. After every epoch of training, we run the policy for 10 test rollouts \emph{where interventions are not allowed} and report the task reward on these rollouts in Figure~\ref{fig:mujoco}. Results suggest that \algabbr is able to match or outperform all baselines in terms of task performance across all simulation environments (Figure~\ref{fig:mujoco}A). Additionally, \algabbr requires far fewer context switches compared to SafeDAgger (Figure~\ref{fig:mujoco}D), while requesting a similar number of supervisor actions across domains (Figure~\ref{fig:mujoco}C): we observe a 79\%, 56\%, and 46\% reduction in context switches on the HalfCheetah, Walker2D, and Ant environments respectively. \algname and SafeDAgger both use an order of magnitude fewer supervisor actions than DAgger. While SafeDAgger requests much fewer supervisor actions than \algname in the Ant environment, this limited amount of supervision is insufficient to match the task performance of \algname or any of the baselines, suggesting that SafeDAgger may be terminating interventions prematurely. We study the total supervisor burden of SafeDAgger and \algname as defined in Equation~\eqref{eq:burden} and find that in HalfCheetah, Walker2D, and Ant, the cutoff latencies $L^*$ are 0.0, 4.3, and 7.6 respectively, i.e. \algname achieves lower supervisor burden in the HalfCheetah domain for any $L$ as well as lower burden in Walker2D and Ant for $L > 4.3$ and $L > 7.6$ respectively. The results suggest that \algname can reduce total supervisor burden compared to SafeDAgger even for modest latency values, but that SafeDAgger may be a better option for settings with extremely low latency.

\textbf{Ablations: } We study 2 key ablations for \algname in simulation: (1) returning to autonomous mode with $\ffilt(\cdot)$ rather than using the ground truth discrepancy (\algname (-Switch to Auto) in Figure~\ref{fig:mujoco}), and (2) removal of noise injection (\algname (-Noise)). \algabbr outperforms both ablations on all tasks, with the exception of ablation 1 on Walker2D, which performed similarly well. We also observe that \algabbr consistently requests more supervisor actions than either ablation. This aligns with the intuition that both using the ground truth action discrepancy to switch back to autonomous mode and injecting noise result in longer but more useful interventions that improve performance. 
% in terms of how costly a context switch is compared to an individual action in Figure~\ref{fig:mujoco}E. \algname has lower overall supervisor burden than SafeDAgger for any switch ratio in HalfCheetah as well as ratios greater than $L = 4.3$ in Walker and $L = 7.6$ in Ant.

%\begin{figure}[tb!]
%\vspace{-0.01in}

% \begin{figure*}[t]
% \center
% \includegraphics[width=0.8\textwidth]{figures/phys-task2.png}
% \caption{
% \textbf{Physical Fabric Manipulation Task: } We evaluate on a 3-stage fabric manipulation task consisting of smoothing a crumpled fabric, aligning the fabric so all corners are visible in the observations, and performing a triangular fold.}
% \label{fig:phystask}
% \end{figure*}
% \vspace{-0.13in}

% \begin{figure}[t]
% \center
% \includegraphics[width=0.45\textwidth]{figures/robotfleetv2.png}
% \caption{
% \textbf{Robot Fleet: } We compare the performance of a robot fleet using \algabbr and SafeDAgger. The y-axis is cumulative reward obtained by 3 robots and the x-axis is the time penalty for a context switch between robots. \algabbr outperforms SafeDAgger on HalfCheetah and Walker for all time penalties as well as Ant for high time penalties.}
% \label{fig:robotfleet}
% \end{figure}
% \textbf{Managing a Robot Fleet: } To compare the performance of \algabbr and SafeDAgger in a robot fleet setting, we re-interpret the MuJoCo simulation experiments as a small robot fleet in Figure~\ref{fig:robotfleet}. Specifically, we assume 1 supervisor and 3 robots, represented by each individual run. Since there is only 1 supervisor, robots requesting assistance must wait in a FIFO queue without making task progress until their intervention request is served. We assume that each action by a robot or supervisor takes 1 timestep, and we apply time penalty $L$ for context switching between robots. We run the fleet for 30,000 timesteps and plot the cumulative reward obtained by all 3 robots in Figure~\ref{fig:robotfleet}. We find that \algabbr obtains higher reward than SafeDAgger for the HalfCheetah fleet and Walker fleet regardless of the context switch penalty, but only outperforms SafeDAgger on Ant for $L > 17$. These results suggest that \algabbr is a more suitable algorithm for supervising a robot fleet if the burden of a context switch is high relative to an individual action. \todo{Clean up this paragraph}

\begin{figure*}[t]
\center
\includegraphics[width=0.90\textwidth]{figures/phystaskandrollouts.png}
\caption{
\textbf{Physical Fabric Manipulation Task: }\textit{Left: } We evaluate on a 3-stage fabric manipulation task consisting of smoothing a crumpled fabric, aligning the fabric so all corners are visible in the observations, and performing a triangular fold. \textit{Right: }  Rollouts of the fabric manipulation task, where each frame is a 100 $\times$ 100 $\times$ 3 overhead image. Human supervisor actions are denoted in red while autonomous robot actions are in green. Rollouts are shaded to indicate task progress: blue for smoothing, red for alignment, and green for folding. SafeDAgger ends human intervention prematurely, resulting in poor task performance and more context switches, while \algname switches back to robot control only when confident in task completion.}
\label{fig:phys-rollouts}
\end{figure*}

\begin{table*}[ht]
%  \begin{center}
\centering
%\resizebox{\columnwidth}{!}
{
 \begin{tabular}{|l | c | c | c | c | c | c | c | c | c | c | c |} 
 \hline
 Algorithm & Task Successes & \multicolumn{3}{c|}{Task Progress} & Context Switches & Supervisor Actions & Robot Actions & \multicolumn{4}{c|}{Failure Modes} \\ 
 \hline
\multicolumn{2}{|c|}{} & (1) & (2) & (3) & \multicolumn{3}{c|}{} & A & B & C & D \\
 \hline
 Behavior Cloning & 0/10 & 6/10 & 0/10 & 0/10 & N/A & N/A & 119 & 2 & 1 & 7 & 0 \\
 \hline
 SD-Execution & 2/10 & 6/10 & 4/10 & 2/10 & 53 & \textbf{34} & 108 & 5 & 0 & 0 & 3 \\
 \hline
 LD-Execution & \textbf{8/10} & 10/10 & 10/10 & 8/10 & \textbf{21} & 43 & 47 & 0 & 0 & 0 & 2 \\
\hline
\end{tabular}}
\caption{\textbf{Physical Fabric Manipulation Experiments:} We evaluate \algname-Execution and baselines on a physical 3-stage fabric manipulation task and report the success rate and supervisor burden in terms of total supervisor actions and bidirectional context switches (summed across all 10 trials). Task Progress indicates how many trials completed each of the 3 stages: Smoothing, Aligning, and Folding. \algname-Execution achieves more successes with fewer context switches ($L^* = 0.28$). We observe the following failure modes (Table~\ref{tab:phys_results}): (A) action limit hit ($>$ 15 total actions), (B) fabric is more than 50\% out of bounds, (C) incorrect predicted pick point, and (D) the policy failed to request an intervention despite high ground truth action discrepancy.}
\label{tab:phys_results}
\end{table*}

\subsection{Fabric Smoothing in Simulation} \label{ssec:fabric_sim_results}
\textbf{Environment: }
We evaluate \algabbr on the fabric smoothing task from~\cite{seita_fabrics_2020} (shown in Figure~\ref{fig:sim2sim}) using the simulation environment from~\cite{seita_fabrics_2020}. The task requires smoothing an initially crumpled fabric and is challenging due to the infinite-dimensional state space and complex dynamics, motivating learning from human feedback. As in prior work~\cite{seita_fabrics_2020}, we utilize top-down $100 \times 100 \times 3$ RGB image observations of the workspace and use actions which consist of a 2D pick point and a 2D pull vector. See~\cite{seita_fabrics_2020} for further details on the fabric simulator.

\textbf{Experimental Setup: }
We train a fabric smoothing policy in simulation using DAgger under supervision from an analytic corner-pulling policy that leverages the simulator's state to identify fabric corners, iterate through them, and pull them towards the corners of the workspace~\cite{seita_fabrics_2020}. We transfer the resulting policy for a 16$\times$16 grid of fabric into a new simulation environment with altered fabric dynamics (i.e. lower spring constant, altered fabric colors, and a higher-fidelity 25$\times$25 discretization) and evaluate \algname and baselines on how rapidly they can adapt the initial policy to the new domain. As in~\cite{seita_fabrics_2020}, we terminate rollouts when we exceed 10 time steps, 92\% coverage, or have moved the fabric more than 20\% out of bounds. We evaluate performance based on a coverage metric, which measures the percentage of the background plane that the fabric covers (fully smooth corresponds to a coverage of 100).

\textbf{Results: }
We report results for the fabric smoothing simulation experiments in Figure~\ref{fig:sim2sim}. Figure~\ref{fig:sim2sim}~(A) shows the performance of the SafeDAgger and \algname policies during learning. To generate this plot we periodically evaluated each policy on \emph{test} rollouts without interventions. Figure~\ref{fig:sim2sim}~(B) and (C) show the number of supervisor actions and context switches required during learning; \algname performs fewer context switches than SafeDAgger but requires more supervisor actions as the interventions are longer. Results suggest that the cutoff latency (as defined in Section~\ref{ssec:metrics}) is $L^*=1.5$ for fabric smoothing. Despite fewer context switches, \algname achieves comparable performance to SafeDAgger, suggesting that \algname can learn complex, high-dimensional robotic control policies while reducing the number of hand-offs to a supervisor. We also evaluate \algname-Execution and SafeDAgger-Execution, in which interventions are allowed but the policy is no longer updated (see Section~\ref{ssec:physresults}). We see that in this case, \algname achieves similar final coverage as SafeDAgger with significantly fewer context switches. 

\subsection{Physical Fabric Manipulation Experiments}\label{ssec:physresults}
\textbf{Environment: }
In physical experiments, we evaluate on a multi-stage fabric manipulation task with an ABB YuMi robot and a human supervisor (Figure~\ref{fig:phys-rollouts}). Starting from a crumpled initial fabric state, the task consists of 3 stages: (1) fully smooth the fabric, (2) align the fabric corners with a tight crop of the workspace, and (3) fold the fabric into a triangular fold. Stage (2) in particular requires high precision, motivating human interventions. As in the fabric simulation experiments, we use top-down $100 \times 100 \times 3$ RGB image observations of the workspace and have 4D actions consisting of a pick point and pull vector. The actions are converted to workspace coordinates with a standard calibration procedure and analytically mapped to the nearest point on the fabric. Human supervisor actions are provided through a point-and-click interface for specifying pick-and-place actions. See the supplement for further details.
% \todo{Ryan: describe the environment here, not how your exp setup works}
% As in prior work~\cite{fabric_vsf,seita_fabrics_2020}, we train a policy with 100 x 100 x 3 RGB image observations in simulation to smooth highly crumpled initial configurations. 
% We study fabric smoothing experiments both in simulation and on an ABB YuMi robot.
% For physical transfer the learned policy to a physical robot with the same domain randomization techniques as~\cite{fabric_vsf,seita_fabrics_2020} and fine-tune the model with a small amount of real data. For this final stage of fine-tuning, we consider 3 strategies: (1) Behavior Cloning, (2) SafeDAgger, and (3) LazyDAgger.

\textbf{Experimental Setup: }
Here we study how interventions can be leveraged to improve the final task performance even at \textit{execution time}, in which policies are no longer being updated. We collect 20 offline task demonstrations and train an initial policy with behavior cloning. To prevent overfitting to a small amount of real data, we use standard data augmentation techniques such as rotating, scaling, changing brightness, and adding noise to create 10 times as many training examples. We then evaluate the behavior cloning agent (Behavior Cloning) and agents which use the SafeDAgger and \algname intervention criteria but do not update the policy with new experience or inject noise (SafeDAgger-Execution and \algname-Execution respectively). We terminate rollouts if the fabric has successfully reached the goal state of the final stage (i.e. forms a perfect or near-perfect dark brown right triangle as in~\citet{fabric_vsf}; see Figure~\ref{fig:phys-rollouts}), more than 50\% of the fabric mask is out of view in the current observation, the predicted pick point misses the fabric mask by approximately 50\% of the plane or more, or 15 total actions have been executed (either autonomous or supervisor).

\textbf{Results: }
We perform 10 physical trials of each technique. In Table~\ref{tab:phys_results}, we report both the overall task success rate and success rates for each of the three stages of the task: (1) Smoothing, (2) Alignment, and (3) Folding. We also report the total number of context switches, supervisor actions, and autonomous robot actions summed across all 10 trials for each algorithm (Behavior Cloning, SafeDAgger-Execution, \algname-Execution). In Figure~\ref{fig:phys-rollouts} we provide representative rollouts for each algorithm. Results suggest that Behavior Cloning is insufficient for successfully completing the alignment stage with the required level of precision. SafeDAgger-Execution does not improve the task success rate significantly due to its inability to collect interventions long enough to navigate bottleneck regions in the task (Figure~\ref{fig:phys-rollouts}). \algname-Execution, however, achieves a much higher success rate than SafeDAgger-Execution and Behavior Cloning with far fewer context switches than SafeDAgger-Execution: \algname-Execution requests 2.1 context switches on average per trial (i.e. 1.05 interventions) as opposed to 5.3 switches (i.e. 2.65 interventions). \algname-Execution trials also make far more task progress than the baselines, as all 10 trials reach the folding stage. \algname-Execution does request more supervisor actions than SafeDAgger-Execution, as in the simulation environments. \algname-Execution also requests more supervisor actions relative to the total amount of actions due to the more conservative switching criteria and the fact that successful episodes are shorter than unsuccessful episodes on average. Nevertheless, results suggest that for this task, \algname-Execution reduces supervisor burden for any $L > L^* = 0.28$, a very low cutoff latency that includes all settings in which a context switch is at least as time-consuming as an individual action (i.e. $L \geq 1$).

In experiments, we find that SafeDAgger-Execution's short interventions lead to many instances of Failure Mode A (see Table~\ref{tab:phys_results}), as the policy is making task progress, but not quickly enough to perform the task. We observe that Failure Mode C is often due to the fabric reaching a highly irregular configuration that is not within the training data distribution, making it difficult for the robot policy to make progress. We find that SafeDAgger and \algname experience Failure Mode D at a similar rate as they use the same criteria to solicit interventions (but different termination criteria). However, we find that all of \algname's failures are due to Failure Mode D, while SafeDAgger also fails in Mode A due to premature termination of interventions.
% For Behavior Cloning, Failure Mode A refers to reaching a significantly off-distribution folded configuration that results in a highly erratic autonomous policy. \todo{add small figure for intuition?} For SafeDAgger-Execution and \algabbr-Execution, Failure Mode A refers to reaching a fabric configuration that is very difficult or impossible for the human supervisor to correct. SafeDAgger-Execution's premature termination of interventions (Figure~\ref{fig:phys-rollouts}) results in more instances of Failure Mode B.


% \todo{note that results worse cuz of harder start states}
% We report Table~\ref{tab:phys_results} for physical trials. We report the number of bidirectional context switches (robot to human and vice versa) as well as the number of supervisor actions for SafeDAgger and \algname over the full 100 time steps of training. We then run 5 trials of Behavior Cloning (BC), SafeDAgger, and \algname and report the average and standard deviation of maximum coverage attained during each trial. During these trials, SafeDAgger and \algname are \textit{not} able to switch to the supervisor as they were during training.
%  \begin{figure}
%      \centering
%      \includegraphics[width=0.48\textwidth]{figures/qualitative.pdf}
%      \caption{Representative policy rollouts on the ABB YuMi for SafeDAgger (top) and \algname (bottom). Human supervisor actions are indicated with red arrows while robot actions are indicated in green. We find that \algname only allows the robot to resume control when confident in task completion, while SafeDAgger ends the intervention prematurely.}
%      \label{fig:lazyvssafe}
%  \end{figure}


==> CASE 2021_ Lazy-DAgger/6-discussion.tex <==
%\vspace{-0.18in}
\section{Discussion and Future Work}
\label{sec:discussion}
We propose context switching between robot and human control as a metric for supervisor burden in interactive imitation learning and present \algname, an algorithm which can be used to efficiently learn tasks while reducing this switching. We evaluate \algname on 3 continuous control benchmark environments in MuJoCo, a fabric smoothing environment in simulation, and a fabric manipulation task with an ABB YuMi robot and find that \algname is able to improve task performance while reducing context switching between the learner and robot by up to 79\% over SafeDAgger. %\ashwin{update with final results}
% \db{briefly say something here about robot fleet?} 
In subsequent work, we investigate more intervention criteria and apply robot-gated interventions to controlling a fleet of robots, where context switching can negatively impact task throughput.
%In future work, we hope to further improve the robustness of the algorithm and apply it to various complex robotic manipulation tasks such as cable untangling and suturing. %\ashwin{update with final results}
%Due to the COVID-19 pandemic, we were unable to perform formal user studies for \algname, and are excited to do this in future work. We will also explore applications and extensions of \algname towards human operators controlling robot fleets, in which the burden of context switching may be even more significant.



==> CASE 2021_ Lazy-DAgger/7-acknowledgement.tex <==
\section{Acknowledgments}
\footnotesize
This research was performed at the AUTOLAB at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab, and the CITRIS ``People and Robots" (CPAR) Initiative. This research was supported in part by the Scalable Collaborative Human-Robot Learning (SCHooL) Project, NSF National Robotics Initiative Award 1734633. The authors were supported in part by donations from Google, Siemens, 
Toyota Research Institute, Autodesk, Honda, Intel, and Hewlett-Packard and by 
equipment grants from PhotoNeo, Nvidia, and Intuitive Surgical. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the sponsors. %Ashwin Balakrishna is supported by an NSF GRFP and Daniel Seita is supported by a Graduate Fellowship for STEM Diversity (GFSD). 
We thank colleagues Lawrence Chen, Jennifer Grannen, and Vincent Lim for providing helpful feedback and suggestions.
